A Newton Frank-Wolfe Method for Constrained Self-Concordant Minimization

We demonstrate how to scalably solve a class of constrained self-concordant minimization problems using linear minimization oracles (LMO) over the constraint set. We prove that the number of LMO calls of our method is nearly the same as that of the Frank-Wolfe method in the L-smooth case. Specifically, our Newton Frank-Wolfe method uses $\mathcal{O}(\epsilon^{-\nu})$ LMO's, where $\epsilon$ is the desired accuracy and $\nu:= 1 + o(1)$. In addition, we demonstrate how our algorithm can exploit the improved variants of the LMO-based schemes, including away-steps, to attain linear convergence rates. We also provide numerical evidence with portfolio design with the competitive ratio, D-optimal experimental design, and logistic regression with the elastic net where Newton Frank-Wolfe outperforms the state-of-the-art.

==> sections/refs.tex <==
\begin{thebibliography}{10}

\bibitem{Bauschke2011}
H.~H. Bauschke and P.~Combettes.
\newblock {\em Convex analysis and monotone operators theory in {H}ilbert
  spaces}.
\newblock Springer-Verlag, 2nd edition, 2017.

\bibitem{Beck2009}
A.~Beck and M.~Teboulle.
\newblock {A} fast iterative shrinkage-thresholding agorithm for linear inverse
  problems.
\newblock {\em SIAM J. Imaging Sci.}, 2(1):183--202, 2009.

\bibitem{Beck2004}
Amir Beck and Marc Teboulle.
\newblock A conditional gradient method with linear rate of convergence for
  solving convex linear systems.
\newblock {\em Mathematical Methods of Operations Research}, 59(2):235--247,
  Jun 2004.

\bibitem{Becker2011a}
S.~Becker, E.~J. Cand\`{e}s, and M.~Grant.
\newblock Templates for convex cone problems with applications to sparse signal
  recovery.
\newblock {\em Math. Program. Compt.}, 3(3):165--218, 2011.

\bibitem{CC01a}
C.-C. Chang and C.-J. Lin.
\newblock {LIBSVM}: {A} library for {S}upport {V}ector {M}achines.
\newblock {\em ACM Transactions on Intelligent Systems and Technology},
  2:27:1--27:27, 2011.

\bibitem{damla2008linear}
S.~A. Damla, P.~Sun, and M.~J. Todd.
\newblock Linear convergence of a modified {F}rank--{W}olfe algorithm for
  computing minimum-volume enclosing ellipsoids.
\newblock {\em Optimisation Methods and Software}, 23(1):5--19, 2008.

\bibitem{SAGA}
A.~Defazio, F.~Bach, and S.~Lacoste-Julien.
\newblock {SAGA}: {A} fast incremental gradient method with support for
  non-strongly convex composite objectives.
\newblock In {\em Advances in Neural Information Processing Systems (NIPS)},
  pages 1646--1654, 2014.

\bibitem{Duchi2008a}
John Duchi, Shai Shalev-Shwartz, Yoram Singer, and Tushar Chandra.
\newblock Efficient projections onto the l1-ball for learning in high
  dimensions.
\newblock In {\em Proceedings of the 25th International Conference on Machine
  Learning}, ICML '08, pages 272--279, New York, NY, USA, 2008. ACM.

\bibitem{Frank1956}
M.~Frank and P.~Wolfe.
\newblock {A}n algorithm for quadratic programming.
\newblock {\em Naval Research Logistics Quarterly}, 3:95--110, 1956.

\bibitem{garber2013linearly}
D.~Garber and E.~Hazan.
\newblock A linearly convergent conditional gradient algorithm with
  applications to online and stochastic optimization, 2013.

\bibitem{garber2015faster}
D.~Garber and E.~Hazan.
\newblock Faster rates for the frank-wolfe method over strongly-convex sets.
\newblock In {\em Proceedings of the 32nd International Conference on Machine
  Learning}, volume 951, pages 541--549, 2015.

\bibitem{gross2010quantum}
D.~Gross, Y.-K. Liu, S.~Flammia, S.~Becker, and J.~Eisert.
\newblock Quantum state tomography via compressed sensing.
\newblock {\em Physical review letters}, 105(15):150401, 2010.

\bibitem{guelat1986some}
J.~Guelat and P.~Marcotte.
\newblock Some comments on wolfe's away step.
\newblock {\em Math. Program.}, 35(1):110--119, 1986.

\bibitem{harman2009approximate}
R.~Harman and M.~Trnovsk\'{a}.
\newblock {A}pproximate {D}-optimal designs of experiments on the convex hull
  of a finite set of information matrices.
\newblock {\em Mathematica Slovaca}, 59(6):693--704, 2009.

\bibitem{Hazan2008}
Elad Hazan.
\newblock Sparse approximate solutions to semidefinite programs.
\newblock In {\em Latin American symposium on theoretical informatics}, pages
  306--316. Springer, 2008.

\bibitem{Jaggi2013}
M.~Jaggi.
\newblock {R}evisiting {F}rank-{W}olfe: {P}rojection-{F}ree {S}parse {C}onvex
  {O}ptimization.
\newblock {\em JMLR W\&CP}, 28(1):427--435, 2013.

\bibitem{Khachiyan1996}
Leonid~G Khachiyan.
\newblock Rounding of polytopes in the real number model of computation.
\newblock {\em Mathematics of Operations Research}, 21(2):307--320, 1996.

\bibitem{lacoste2015global}
S.~Lacoste-Julien and M.~Jaggi.
\newblock On the global linear convergence of {F}rank-{W}olfe optimization
  variants.
\newblock In {\em Advances in Neural Information Processing Systems}, pages
  496--504, 2015.

\bibitem{lan2016conditional}
G.~Lan and Y.~Zhou.
\newblock Conditional gradient sliding for convex optimization.
\newblock {\em SIAM J. Optim.}, 26(2):1379--1409, 2016.

\bibitem{lan2016accelerated}
Guanghui Lan and Yuyuan Ouyang.
\newblock Accelerated gradient sliding for structured convex optimization.
\newblock {\em Arxiv preprint:1609.04905}, 2016.

\bibitem{lu2013computing}
Z.~Lu and T.K. Pong.
\newblock Computing optimal experimental designs via interior point method.
\newblock {\em SIAM J. Matrix Anal. Appl.}, 34(4):1556--1580, 2013.

\bibitem{Nesterov2004}
Y.~Nesterov.
\newblock {\em {I}ntroductory lectures on convex optimization: {A} basic
  course}, volume~87 of {\em Applied Optimization}.
\newblock Kluwer Academic Publishers, 2004.

\bibitem{Nesterov1994}
Y.~Nesterov and A.~Nemirovski.
\newblock {\em Interior-point Polynomial Algorithms in Convex Programming}.
\newblock Society for Industrial Mathematics, 1994.

\bibitem{odor2016frank}
G.~Odor, Y.-H. Li, A.~Yurtsever, Y.-P. Hsieh, Q.~Tran-Dinh, M.~El-Halabi, and
  V.~Cevher.
\newblock {F}rank-{W}olfe works for non-lipschitz continuous gradient
  objectives: {S}calable poisson phase retrieval.
\newblock In {\em 2016 IEEE International Conference on Acoustics, Speech and
  Signal Processing (ICASSP)}, pages 6230--6234. IEEE, 2016.

\bibitem{Ostrovskii2018}
D.~M. Ostrovskii and F.~Bach.
\newblock {F}inite-sample {A}nalysis of {M}-estimators using
  {S}elf-concordance.
\newblock {\em Arxiv preprint:1810.06838v1}, 2018.

\bibitem{peyre2019computational}
G.~Peyr{\'e} and M.~Cuturi.
\newblock Computational optimal transport.
\newblock {\em Foundations and Trends{\textregistered} in Machine Learning},
  11(5-6):355--607, 2019.

\bibitem{ryu2014stochastic}
E.~K. Ryu and S.~Boyd.
\newblock Stochastic proximal iteration: a non-asymptotic improvement upon
  stochastic gradient descent.
\newblock {\em Author website, early draft}, 2014.

\bibitem{Su2014}
W.~Su, S.~Boyd, and E.~Candes.
\newblock A differential equation for modeling {N}esterov's accelerated
  gradient method: {T}heory and insights.
\newblock In {\em Advances in Neural Information Processing Systems (NIPS)},
  pages 2510--2518, 2014.

\bibitem{SunTran2017gsc}
T.~Sun and Q.~Tran-Dinh.
\newblock {G}eneralized {S}elf-{C}oncordant {F}unctions: {A} {R}ecipe for
  {N}ewton-{T}ype {M}ethods.
\newblock {\em Math. Program. (online first)}, pages 1--63, 2018.

\bibitem{Tran-Dinh2013a}
Q.~Tran-Dinh, A.~Kyrillidis, and V.~Cevher.
\newblock Composite self-concordant minimization.
\newblock {\em J. Mach. Learn. Res.}, 15:374--416, 2015.

\bibitem{TranDinh2017d}
Q.~Tran-Dinh, L.~Ling, and K.-C. Toh.
\newblock A new homotopy proximal variable-metric framework for composite
  convex minimization.
\newblock {\em Tech. Report (UNC-STOR)}, pages 1--28, 2018.

\bibitem{TranDinh2016c}
Q.~Tran-Dinh, T.~Sun, and S.~Lu.
\newblock Self-concordant inclusions: A unified framework for path-following
  generalized {N}ewton-type algorithms.
\newblock {\em Math. Program.}, 177(1--2):173--223, 2019.

\bibitem{Yurtsever2015}
A.~Yurtsever, Q.~Tran-Dinh, and V.~Cevher.
\newblock A universal primal-dual convex optimization framework.
\newblock {\em Advances in Neural Information Processing Systems (NIPS)}, pages
  1--9, 2015.

\bibitem{yurtsever2019conditional}
Alp Yurtsever, Olivier Fercoq, and Volkan Cevher.
\newblock A conditional gradient-based augmented lagrangian framework.
\newblock {\em arXiv preprint arXiv:1901.04013}, 2019.

\end{thebibliography}

